SROS2: Usable Cyber Security Tools for ROS 2

ROS 2 is rapidly becoming a standard in the robotics industry. Built upon DDS as its default communication middleware and used in safety-critical scenarios, adding security to robots and ROS computational graphs is increasingly becoming a concern. The present work introduces SROS2, a series of developer tools and libraries that facilitate adding security to ROS 2 graphs. Focusing on a usability-centric approach in SROS2, we present a methodology for securing graphs systematically while following the DevSecOps model. We also demonstrate the use of our security tools by presenting an application case study that considers securing a graph using the popular Navigation2 and SLAM Toolbox stacks applied in a TurtleBot3 robot. We analyse the current capabilities of SROS2 and discuss the shortcomings, which provides insights for future contributions and extensions. Ultimately, we present SROS2 as usable security tools for ROS 2 and argue that without usability, security in robotics will be greatly impaired.

==> body/5.analysis.tex <==
\section{Analysis}
\label{sec:analysis}


\begin{itemize}

    \item best practices applied
        \item separation of concerns (optional)
        \item principle of least privilege (optional)
    \item retrospect on decisions made
        \item driven by application limitations
        \item driven by tooling limitations
        
    \subsection{sec considerations}
    \item vulnerability scanning
    \item CVEs between DDS/RTPS vendors
    
    \subsection{}
    \item access control
    \item information flow control
    \item observability
    \item controllability
    \item tf
  
\end{itemize}

==> figs/diagrams/methodology.tex <==
\begin{figure}[!h]
    \centering
    \scalebox{0.6}{
        \tikzset{
              state1/.style={fill=gray!5},
              state2/.style={fill=gray!1},
              state3/.style={fill=gray!40},
        }    
        \begin{tikzpicture}[shorten >=1pt,node distance=5cm,on grid,auto]
          \tikzstyle{every state}=[fill={rgb:black,1;white,10}]
        
            \node[state,initial, state3]    (q_1)                    {A. Modeling};
            \node[state, state1]            (q_2)  [right of=q_1]    {B. Authentication};
            \node[state, state1]            (q_3)  [right of=q_2]    {C. Authorization};
            \node[state, state1]            (q_4)  [above of=q_3]    {D. Generation};
            \node[state, state1]            (q_5)  [left of=q_4]     {E. Deployment};
            \node[state, state1]            (q_6)  [left of=q_5]     {F. Monitoring};
        
            \path[->]
                (q_1) edge [right] node { }    (q_2)
                (q_2) edge [right] node { }    (q_3)
                (q_3) edge [bend right] node { }    (q_4)
                (q_4) edge [right] node { }    (q_5)
                (q_5) edge [right] node { }    (q_6)
                (q_6) edge [loop above] node {}   (   );
            \path[->, dashed]
                (q_6) edge [bend right] node { }    (q_1);

        \end{tikzpicture}}
    \caption{\textbf{Our methodology for securing ROS 2 computational graphs}. SROS2 provides tools and libraries to facilitate a secure DevOps model in robotics (DevSecOps \cite{mayoral2020devsecops}).} 
    %by (1) providing tools to introspect and model the graph, allow to configure (2) authentication and (3) authorization, (4) generation of the security artifacts, (5) deployment and (6) continuous monitoring.}
    \label{fig:methodology}
\end{figure}


==> figs/diagrams/monitoring.tex <==
\lstset{language=bash}
\lstset{label={lst:monitoring}}
\lstset{basicstyle=\ttfamily\footnotesize,
    commentstyle=\color{MidnightBlue}}
\lstset{caption={SROS2 provides tools to dissect DDS interactions, extract key information and map it to outstanding security flaws affecting DDS.} 
}
\lstset{escapeinside={<@}{@>}}
\begin{lstlisting}
# monitor the network segment for vulnerabilities affecting DDS participants
ros2 security monitor
<@\textcolor{gray}{sniffing the DDS network...}@>
<@\textcolor{RedViolet}{Vulnerable DDS endpoint found (hostId=16974402, appId=2886795267, instanceId=10045242)}@>
    <@\textcolor{RedViolet}{- vendorId: Real-Time Innovations, Inc. - Connext DDS}@>
    <@\textcolor{RedViolet}{- version: 6.0.1.25}@>
    <@\textcolor{RedViolet}{- CVE IDs:}@>
        <@\textcolor{RedViolet}{* CVE-2021-38487}@>
        <@\textcolor{RedViolet}{* CVE-2021-38435}@>
\end{lstlisting}

==> figs/diagrams/navigationgraph.tex <==
\begin{figure*}[t]
    \centering
    %\includegraphics[width=1.0\textwidth]{figs/diagrams/graph2.png}
    \includegraphics[width=1.0\textwidth]{figs/diagrams/graph3.png}
    \caption{\textbf{A simulated TurtleBot3 secured using SROS2}. The figure depicts a subset of the computational graph of the robot including sensor and control topics as well some relevant portions of the \texttt{slam\_toolbox} and \texttt{navigation2} software stacks.}
    \label{fig:navigationgraph}
\end{figure*}


==> figs/diagrams/rosgraph/old.rosgraph.tex <==
% Filtered Nodes 
% -/gazebo.*,-/transform.*,-/lifecycle.*,-/.*_imu, -/local_costmap_client, -/recoveries_server_rclcpp_node, -/global_costmap_client,-/.*transform_listener.*
% Filtered Topics
% -/bond,-/.*/status,-/waypoints
% Group: all but tf
% Hidden: all but tf

\begin{figure*}[!htb]
    \centering
    \includegraphics[
        width=\linewidth,
        trim= 0 300 1500 0,
        clip
        ]
        {figs/diagrams/rosgraph/rosgraph.pdf}
    \caption{\textbf{A portion of the simulated TurtleBot3 secured using SROS2}. The figure depicts a subset of the computational graph of the robot including sensor and control topics as well some relevant portions of the \texttt{navigation2} software stack.}
    \label{fig:navigationgraph}
\end{figure*}
